Fast and Robust Localization for Humanoid Soccer Robot via Iterative Landmark Matching

Accurate robot localization is essential for effective operation. Monte Carlo Localization (MCL) is commonly used with known maps but is computationally expensive due to landmark matching for each particle. Humanoid robots face additional challenges, including sensor noise from locomotion vibrations and a limited field of view (FOV) due to camera placement. This paper proposes a fast and robust localization method via iterative landmark matching (ILM) for humanoid robots. The iterative matching process improves the accuracy of the landmark association so that it does not need MCL to match landmarks to particles. Pose estimation with the outlier removal process enhances its robustness to measurement noise and faulty detections. Furthermore, an additional filter can be utilized to fuse inertial data from the inertial measurement unit (IMU) and pose data from localization. We compared ILM with Iterative Closest Point (ICP), which shows that ILM method is more robust towards the error in the initial guess and easier to get a correct matching. We also compared ILM with the Augmented Monte Carlo Localization (aMCL), which shows that ILM method is much faster than aMCL and even more accurate. The proposed method's effectiveness is thoroughly evaluated through experiments and validated on the humanoid robot ARTEMIS during RoboCup 2024 adult-sized soccer competition.

==> Sections/S0_nomenclature.tex <==
%%% Section needed to define variables

\nomenclature{$p$}{probability of latching success for a position.}
\nomenclature{$r$}{length from cutout center to nearest hole edge.}
% \nomenclature{$r'$}{length from assembly center to cutout center.}
\nomenclature{$R$}{radial length of cutout.}
\nomenclature{$\rho$}{length from blade assembly center to blade tips.}
\nomenclature{$\tau$, $u$}{torque and control input, respectively.}
% \nomenclature{$\theta$}{angle between $r'$ and nearest edge.}
\nomenclature{$\omega$}{orientation misalignment between latch and pattern.}
\nomenclature{$\vartheta$}{angle between edges defining holes in pattern.}
\nomenclature{$W$}{length from blade assembly center to outer limit.}
\nomenclature{$x$, $y$}{Cartesian coordinates of $r$ and $\theta$.}
\nomenclature{*}{indicates an optimal parameter.}
\nomenclature{$\Psi$}{misalignment tolerance metric.}
\nomenclature{$h$}{height from tips of blades to base.}
\nomenclature{$q$, $\dot{q}$, $\ddot{q}$}{joint angle, velocity, and acceleration, respectively.}
\nomenclature{$K$, $M$}{joint controller gains and mass matrix, respectively.}
\nomenclature{$c$, $g$, $b$}{Coriolis, gravity, and damping terms, respectively.}
\nomenclature{$J$, $F$}{Jacobian and end effector forces, respectively.}

\printnomenclature

==> Sections/S2_data_assignment.tex <==

\section{Data Association}
\label{sec:data_associ}

% problem definition:
Our approach requires us to first match the landmarks to its observations from the camera with the landmarks in the apriori known map, the soccer field. Our stereo vision system will detect landmarks, such as corners, t-intersections, crosses, and goal posts, relative to the robot. Matching the landmarks with positional information is a typical Linear Assignment Problem (LAP). 

Different kind of landmarks can be matched separately considering their classification or treated identically as shown in \cref{fig:Landmark_matching}. Matching different kinds separately makes the matching more accurate when the classification is correct. However, if some landmarks are misclassified, it will be less accurate. Therefore, we use two methods in parallel and choose the result with less error. 

% \FloatBarrier

\begin{figure*}[htbp]
% \begin{figure*}[h!]
% \begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\linewidth]{Figures/S2_data_assignment/good_matching_by_good_classification_crop.png}
        \caption{Matching landmarks separately, no misclassification.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\linewidth]{Figures/S2_data_assignment/mismatching_by_not_using_classification_crop.png}
        \caption{Matching landmarks identically, no misclassification.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\linewidth]{Figures/S2_data_assignment/mismatching_by_miss_classification_crop.png}
        \caption{Matching landmarks separately with misclassification.}
    \end{subfigure}
    
    \caption{Landmark matching under different scenarios. This mismatched landmarks are circled in yellow. (a) shows the correct matching. (b) shows the mismatching due to treat different kind of landmarks identically (c) shows the mismatching due to misclassification}
    \label{fig:Landmark_matching}
\end{figure*}


The common methods for solving LAP are Kuhn–Munkres algorithm (Hungarian algorithm) \cite{kuhn1955hungarian,munkres1957algorithms}, Jonker-Volgenant algorithm \cite{jonker1988shortest}, and integer linear programming \cite{selmair2021evaluation}. We also note multiple improvements and modifications of the Jonker-Volgenant algorithm \cite{malkoff1997evaluation,crouse2016implementing}. In the case that the number of data points is large, like when using LiDAR, nearest neighbour (NN) is also good for lower computational complexity \cite{bentley1975multidimensional,friedman1977algorithm,arya1998optimal}. There are also papers comparing the performance of methods \cite{selmair2021evaluation,levedahl2000performance}.
% how to solve::

For our case, the number of points are small, so what matters is to guarantee the optimal solution in a fast enough time for real time localization applications. Therefore, Kuhn–Munkres algorithm \cite{munkres1957algorithms}, Jonker-Volgenant algorithm \cite{jonker1988shortest} and the modified Jonker-Volgenant algorithm \cite{crouse2016implementing} are good candidates to use to solve LAP for our localization method. 

We simulated the soccer field and timed the three methods by randomly sampling 100,000 poses on the field uniformly. The results in  \cref{fig:matching_time_10000} shows that the modified Jonker-Volgenant algorithm \cite{crouse2016implementing} is the fastest with a high rate of consistency. Therefore, we chose this method to match our landmarks. 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/S2_data_assignment/matching_time_10000.png}
%     \caption{The solve time for three methods solving LAP.}
%     \label{fig:matching_time_10000}
% \end{figure}

% \begin{table}[h!]
% \centering
% \caption{The average calculation time for data assignment in millisecond}
% \label{tab:data_assignment_time_in_ms}
% \begin{tabular}{|c|c|c|}
% \hline
% Kuhn–Munkres & Jonker-Volgenant & modified Jonker-Volgenant \\
% \hline
% 0.583 ms & 0.0570 ms & 0.0381 ms \\
% \hline
% \end{tabular}
% \end{table}




==> Sections/S3_pose_estimation_by_damped_least_square.tex <==
\section{Pose Estimation}
\label{sec:pose_esti}
% problem definition:
% \subsection{problem definition}
The next component of our localization estimates the 2D pose according to the matched landmarks from \cref{sec:data_associ}. The 2D pose of a robot includes the position (x,y) and orientation $\theta$. There are several methods that solve this including nonlinear programming (NLP), Direct Linear Transformation (DLT), and the Kabsch algorithm \cite{kabsch1976solution,arun1987least,maurer1996registration}. The nonlinear programming method is flexible, handling various types of transformations and constraints. However, the methods for NLP like Sequential Quadratic Programming, Interior-Point Method, and Levenberg-Marquardt method, are computationally expensive. Moreover, NLP might give a local optimal as a solution which can be detrimental for our use case. The DLT method and Kabsch algorithm give close form solutions \cite{kabsch1976solution,arun1987least,maurer1996registration} for the 2D pose which is faster and better meets our needs.

% The problem is formulated as following.
Given a set of points in the body frame $p^{\text{body}}_{\text{i}}$ and the corresponding points in the world frame $p^{\text{world}}_{\text{i}}$, we need to find the 2D transformation \((t_x,t_y,\theta)\) which maps the body frame points to the world frame points.
We define the translation vector as $t = (t_{x},t_{y})$, and the rotation angle as $\theta$. The transformation can be expressed as:
\begin{equation*}
p^{\text{world}}_{\text{i}} = R(\theta) \cdot p^{\text{body}}_{\text{i}}+ t
\label{eq:2D_transformation}
\end{equation*}
where $R(\theta)$ is a 2D rotation matrix:
\begin{equation*}
R(\theta) = \begin{pmatrix} 
\cos(\theta) & -\sin(\theta) \\ 
\sin(\theta) & \cos(\theta) 
\end{pmatrix}
\label{eq:rotation_matrix}
\end{equation*}

% \[
% R(\theta) = \begin{pmatrix} \cos\theta & -\sin\theta \\ \sin\theta & \cos\theta \end{pmatrix}
% \]




% method 1 :: solve by linear method ::
\subsection{Direct Linear Transformation}
The 2D transformation from the body frame to the world frame can be described by the following equations:
\begin{align*}
x_i^{\text{world}} &= \cos(\theta) x_i^{\text{body}} - \sin(\theta) y_i^{\text{body}} + t_x \\
y_i^{\text{world}} &= \sin(\theta) x_i^{\text{body}} + \cos(\theta) y_i^{\text{body}} + t_y
\end{align*}
This can be rewritten in a linear form:
\begin{equation*}
\begin{pmatrix}
    x_i^{\text{body}} & -y_i^{\text{body}} & 1 & 0 \\ 
    y_i^{\text{body}} & x_i^{\text{body}} & 0 & 1 \\ 
\end{pmatrix}
\begin{pmatrix}
    m_1 \\ 
    m_2 \\ 
    m_3 \\
    m_4 \\
\end{pmatrix}
% \begin{pmatrix}
%     \cos(\theta) \\ 
%     \sin(\theta) \\ 
%     t_x \\
%     t_y \\
% \end{pmatrix}
 = 
 \begin{pmatrix}
    x_i^{\text{world}} \\ 
    y_i^{\text{world}} \\ 

\end{pmatrix}
\end{equation*}
where $m_1 = \cos(\theta),m_2 = \sin(\theta),m_3 = t_x,m_4 = t_y$.
% \begin{align*}
% m_1 &= \cos(\theta) \\
% m_2 &= \sin(\theta) \\
% m_3 &= t_x \\
% m_4 &= t_y.
% \end{align*}

For all n points, we can arrange the equations into the following linear form:
\begin{equation*}
\begin{pmatrix}
x_1^{\text{body}} & -y_1^{\text{body}} & 1 & 0 \\
y_1^{\text{body}} & x_1^{\text{body}} & 0 & 1 \\
\vdots & \vdots & \vdots & \vdots \\
x_n^{\text{body}} & -y_n^{\text{body}} & 1 & 0 \\
y_n^{\text{body}} & x_n^{\text{body}} & 0 & 1 \\
\end{pmatrix}
\begin{pmatrix}
m_1 \\
m_2 \\
m_3 \\
m_4 \\
\end{pmatrix}
=
\begin{pmatrix}
x_1^{\text{world}} \\
y_1^{\text{world}} \\
\vdots \\
x_n^{\text{world}} \\
y_n^{\text{world}}
\end{pmatrix}.
\end{equation*}
The system can be written in the form \( A \mathbf{m} = \mathbf{b} \), where:
\begin{itemize}
    \item \( A \) is the matrix constructed from the coordinates in body frame \( (x_i^{\text{body}}, y_i^{\text{body}}) \).
    \item \( \mathbf{m} \) is the vector of unknowns \( (\cos(\theta), \sin(\theta), t_x, t_y) \).
    \item \( \mathbf{b} \) is the vector of matched coordinates in world frame \( (x_i^{\text{world}}, y_i^{\text{world}}) \).
\end{itemize}
Solving for \( \mathbf{m} \) using the least squares method:
\begin{equation*}
\mathbf{m} = (A^T A)^{-1} A^T \mathbf{b}.
\end{equation*}
% Once the linear system is solved, extract the pose parameters as follows:
% \begin{align*}
% \theta &= \text{arctan2}( m_2, m_1) \\
% t_x &= m_3 \\
% t_y &= m_4 \\
% \end{align*}
Then we get the pose parameters: $\theta = \text{arctan2}( m_2, m_1)$, $t_x = m_3$ and $t_y = m_4$.

% \(\theta = \text{arctan2}(m_2, m_1), \; t_x = m_3, \; t_y = m_4\)

% \(\theta &= \text{arctan2}( m_2, m_1),
% t_x &= m_3
% t_y &= m_4 \)



% method 2 :: solve by svd, least square :: 
\subsection{Kabsch Algorithm}
The objective of the Kabsch algorithm is to find the rotation $\theta$ and translation $t$ that minimizes the sum of squared errors between the transformed points and the world frame points:
\begin{equation*}
\min_{\theta, t} \sum_{i=1}^{n} \left\| p^{\text{world}}_{i} - \left( R(\theta) \cdot p^{\text{body}}_{i} + t \right) \right\|^2
\label{eq:optimization}
\end{equation*}
First step is to compute the centroids of the point sets:
\begin{equation*}
\bar{p}^{\text{body}} = \frac{1}{n} \sum_{i=1}^n p_i^{\text{body}}, \quad \bar{p}^{\text{world}} = \frac{1}{n} \sum_{i=1}^n p_i^{\text{world}}.
\end{equation*}
Then subtract the centroids from the corresponding points to create centered point sets:
\begin{equation*}
q_i^{\text{body}} = p_i^{\text{body}} - \bar{p}^{\text{body}}, \quad q_i^{\text{world}} = p_i^{\text{world}} - \bar{p}^{\text{world}}.
\end{equation*}
Next, compute the cross-covariance matrix \( H \), which captures the relationship between the centered point sets:
\begin{equation*}
H = \sum_{i=1}^n q_i^{\text{body}} (q_i^{\text{world}})^T.
\end{equation*}
Then, we use singular value decomposition (SVD) on the cross-covariance matrix \( H \):
\begin{equation*}
H = U \Sigma V^T
\end{equation*}
% Where:
% \begin{itemize}
%     \item \( U \) and \( V \) are \( 2 \times 2 \) orthogonal matrices.
%     \item \( \Sigma \) is a diagonal matrix containing the singular values.
% \end{itemize}
The optimal rotation matrix \( R \) is obtained by multiplying the matrices \( V \) and \( U^T \):
% $R = V U^T$
\begin{equation*}
R = V U^T
\end{equation*}


After computing \( R \), there is a probability that it is a reflection matrix rather than rotation matrix. We should check the determinant to ensure it is a proper rotation matrix:
% \begin{itemize}
%     \item If \( \text{det}(R) = 1 \), \( R \) is a proper rotation matrix.
%     \item If \( \text{det}(R) = -1 \), then \( R \) represents a reflection. In this case, modify \( R \) to make it a proper rotation matrix by flipping the sign of the last column of \( V \) and recomputing \( R \).
% \end{itemize}
% % \hl{Do we need this rotation stuff? - the other paper says yes}


If \( \text{det}(R) = -1 \), adjust \( V \) by $V' = \begin{pmatrix} V_{[:,1]} & -V_{[:,2]} \end{pmatrix}$.
% If \( \text{det}(R) = -1 \), adjust \( V \) as follows:
% \begin{equation*}
% V' = \begin{pmatrix} V_{[:,1]} & -V_{[:,2]} \end{pmatrix}.
% \end{equation*}
Recompute the rotation matrix by $R = V' U^T$.


% Recompute the rotation matrix:
% \begin{equation*}
% R = V' U^T.
% \end{equation*}

Finally, the translation vector \( t = (t_x, t_y) \) is obtained by aligning the centroids after applying the rotation:
\begin{equation*}
t = \bar{p}^{\text{world}} - R \bar{p}^{\text{body}}.
\end{equation*}

\subsection{Comparing}
We calculate the average solving time for the DLT method and Kabsch algorithm in  \cref{fig:pose_estimating_time}. DLT is slightly faster.


% \begin{table}[h!]
% \centering
% \caption{The average calculation time for 2D pose estimation in millisecond}
% \label{tab:pose_estimating_time}
% \begin{tabular}{|c|c|}
% \hline
% Direct Linear Transformation(DLT) & Kabsch algorithm \\
% \hline
% 0.901 ms & 1.132 ms  \\
% \hline
% \end{tabular}
% \end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/pose_estimation_time_10000.png}
    \caption{Average calculation time for 2D pose estimation in milliseconds.}
    \label{fig:pose_estimating_time}
\end{figure}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/xy_error_vs_noise_width.png}
%     \caption{average error in position and orientation considering different level of noise.}
%     \label{fig:pose_estimating_error}
% \end{figure}

% \begin{figure*}[htbp]
%     \centering
%     \begin{subfigure}{0.45\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/xy_error_vs_noise_width.png}
%         \caption{Image A}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.45\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/theta_error_vs_noise_width.png}
%         \caption{Image B}
%     \end{subfigure}

%     \vspace{0.5cm}

%     \begin{subfigure}{0.45\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/distance_vs_noise_width.png}
%         \caption{Image C}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{0.45\textwidth}
%     %     \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/time_vs_noise_width.png}
%     %     \caption{Image D}
%     % \end{subfigure}
    
%     \caption{A 2x2 Grid of Images}
%     \label{fig:2x2grid}
% \end{figure*}

% \begin{figure*}[htbp]
%     \centering
%     \begin{subfigure}{0.25\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/xy_error_vs_noise_width.png}
%         \caption{Image A}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.25\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/theta_error_vs_noise_width.png}
%         \caption{Image B}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.25\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/distance_vs_noise_width.png}
%         \caption{Image C}
%     \end{subfigure}

%     \caption{A 2x2 Grid of Images}
%     \label{fig:2x2grid}
% \end{figure*}


\cref{fig:pose_estimating_error} shows the average error in position and orientation considering different level of noise by uniformly random sampling 100,000 poses on the field. It shows that the Kabsch algorithm has smaller position error than DLT. The orientation errors are the same. Though both methods have their advantage, Kabsch method has a obviously smaller position error and therefore preferred.
% \hl{what's the conclusion? Do we choose DLT or Kabsch?}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/xy_error_vs_noise_width.png}
        % \caption{Image A}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/theta_error_vs_noise_width.png}
        % \caption{Image B}
    \end{subfigure}

    \caption{Average pose estimation error in position and orientation considering different levels of noise.}
    \label{fig:pose_estimating_error}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{0.24\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/xy_error_vs_noise_width.png}
%         % \caption{Image A}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/theta_error_vs_noise_width.png}
%         % \caption{Image B}
%     \end{subfigure}

%     \caption{average error in position and orientation considering different level of noise.}
%     \label{fig:pose_estimating_error}
% \end{figure}



% \begin{figure*}[htbp]
%     \centering
%     \begin{subfigure}{0.3\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/xy_error_vs_noise_width.png}
%         % \caption{Image A}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/theta_error_vs_noise_width.png}
%         % \caption{Image B}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\textwidth}
%         \includegraphics[width=\linewidth]{Figures/S3_pose_estimation_by_damped_least_square/noise_to_pose_error_combine/distance_vs_noise_width.png}
%         % \caption{Image C}
%     \end{subfigure}
    
%     \caption{average error in position and orientation considering different level of noise.}
%     \label{fig:pose_estimating_error}
% \end{figure*}





==> Sections/S5_data_fusion.tex <==
\section{data fusion}
\label{sec:data_fusion}
In the competition, rules allowed for only a single IMU and camera. Two common methods to fuse IMU data with localized estimates are Extended Kalman Filter (EKF) \cite{kim2008accurate} and Particle Filter (PF) \cite{chen2010particle,tariq20242d}. 

% When our robot gets new data from the IMU, it processes a prediction step. When ILM calculates the 2D pose from new vision data, it should process an update step \hl{What does this mean?}. 


Define the state vector \(X\) of the robot in 2D space and control input \(u\) as:
\begin{align*}
\mathbf{X_k} & :=
\begin{bmatrix}
x_k \\
y_k \\
\theta_k
\end{bmatrix}
&
\mathbf{u_k} & :=
\begin{bmatrix}
v_{xk} \\
v_{yk} \\
\omega_{k}
\end{bmatrix}
\end{align*}
% Define the state vector $\mathbf{x}$ of the robot in 2D space is given by:
% \[
% \mathbf{x} = \begin{bmatrix}
% x \\
% y \\
% \theta
% \end{bmatrix}
% \]
where $x$ and $y$ represent the position of the robot, and $\theta$ represents its orientation.
% The control input vector $\mathbf{u}$ is:
% \[
% \mathbf{u} = \begin{bmatrix}
% v \\
% \omega
% \end{bmatrix}
% \]
$v_x$ is the forward velocity, $v_y$ is the lateral velocity and $\omega$ is the angular velocity.
The continuous-time dynamics of the robot can be described by the following nonlinear equations:
% \[
% \dot{\mathbf{x}} = \begin{bmatrix}
% \dot{x} \\
% \dot{y} \\
% \dot{\theta}
% \end{bmatrix}
% = \begin{bmatrix}
% v \cos(\theta) \\
% v \sin(\theta) \\
% \omega
% \end{bmatrix}
% \]
\begin{equation*}
\begin{bmatrix}
\dot{x} \\
\dot{y} \\
\dot{\theta}
\end{bmatrix}
=
\begin{bmatrix}
\cos(\theta) & -\sin(\theta) & 0 \\
\sin(\theta) & \cos(\theta) & 0 \\
 0 & 0 & 1
\end{bmatrix}
\begin{bmatrix}
v_x \\
v_y \\
\omega
\end{bmatrix}
\end{equation*}
where $\dot{x}$, $\dot{y}$, and $\dot{\theta}$ represent the time derivatives of $x$, $y$, and $\theta$, respectively.
For discrete-time implementation, assuming a time step $\Delta t$, the state update equations become:
% \[
% \mathbf{x}_{k+1} = \mathbf{x}_k + \begin{bmatrix}
% v_k \cos(\theta_k) \Delta t \\
% v_k \sin(\theta_k) \Delta t \\
% \omega_k \Delta t
% \end{bmatrix}
% + \mathbf{w}_k
% \]
\begin{equation*}
\mathbf{X}_{k+1} = \mathbf{X}_k 
+
\begin{bmatrix}
\cos(\theta_{k}) & -\sin(\theta_{k}) & 0 \\
\sin(\theta_{k}) & \cos(\theta_{k}) & 0 \\
 0 & 0 & 1
\end{bmatrix}
\begin{bmatrix}
v_x \\
v_y \\
\omega
\end{bmatrix}
\Delta t
+
W_k
\end{equation*}
where $\mathbf{w}_k$ represents the process noise.
The measurement model is $\mathbf{z}_{k} = \mathbf{x}_k + \mathbf{v}_k $, since ILM gives the $\mathbf{x}$ directly.
Since the measurement model is linear and the dynamic model is weakly nonlinear, both EKF \cite{kim2008accurate} and PF \cite{chen2010particle,tariq20242d} work. \cref{alg:pf} shows the particle filter, we used in the RoboCup 2024 competition. 



% \begin{algorithm}
% \caption{Data Fusion by Extended Kalman Filter}
% \label{alg:ekf}
% \begin{algorithmic}[1]
%     \State \textbf{Input:} Initial State estimate $\hat{\mathbf{x}}_0$, initial covariance $P_0$
%     \State \textbf{Output:} Estimated State $\hat{\mathbf{x}}_k$, covariance $P_k$
%     \For{each time step $k$}
%         \State \textbf{Prediction Step:}
%         \State Predict the State: $\hat{\mathbf{x}}_{k|k-1} = \mathbf{f}(\hat{\mathbf{x}}_{k-1}, \mathbf{u}_{k-1})$
%         \State Compute the Jacobian: $F_{k-1} = \frac{\partial \mathbf{f}(\mathbf{x}, \mathbf{u})}{\partial \mathbf{x}} \bigg|_{\hat{\mathbf{x}}_{k-1}, \mathbf{u}_{k-1}}$
%         \State Predict the covariance: $P_{k|k-1} = F_{k-1} P_{k-1} F_{k-1}^T + Q$

%         \State \textbf{Update Step:}
%         \State Compute the predicted measurement: $\hat{\mathbf{z}}_k = \hat{\mathbf{x}}_{k|k-1}$
%         \State $H_k = eye(3)$
%         \State Compute the Kalman gain: $K_k = P_{k|k-1} H_k^T \left( H_k P_{k|k-1} H_k^T + R \right)^{-1}$
%         \State Update the State estimate: $\hat{\mathbf{x}}_k = \hat{\mathbf{x}}_{k|k-1} + K_k \left( \mathbf{z}_k - \hat{\mathbf{z}}_k \right)$
%         \State Update the covariance estimate: $P_k = \left( I - K_k H_k \right) P_{k|k-1}$
%     \EndFor
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{Data Fusion by Particle Filter}
\label{alg:pf}
\begin{algorithmic}[1]
    \State \textbf{Input:} Initial particles $\{\mathbf{x}_i^{(0)}\}_{i=1}^N$ and weights $w_i^{(0)} = \frac{1}{N}$
    \State \textbf{Output:} Estimated State $\hat{\mathbf{x}}^{(t)}$
    \For{each time step $t$}
        \State \textbf{Prediction Step:}
        \For{each particle $i$}
            \State Predict the State: $\mathbf{x}_i^{(t)} = \mathbf{f}(\mathbf{x}_i^{(t-1)}, \mathbf{u}_t) + \mathbf{w}_i$
        \EndFor

        \State \textbf{Update Step:}
        \For{each particle $i$}
            \State Compute the weight: $w_i^{(t)} \propto p(\mathbf{z}_t | \mathbf{x}_i^{(t)})$
        \EndFor

        \State Normalize the weights: $w_i^{(t)} = \frac{w_i^{(t)}}{\sum_{j=1}^{N} w_j^{(t)}}$

        \State \textbf{Resampling:}
        \State Compute effective sample size: $N_{\text{eff}} = \frac{1}{\sum_{i=1}^{N} (w_i^{(t)})^2}$
        \If{$N_{\text{eff}} < \frac{N}{2}$}
            \State  Resampling using \textbf{Systematic Resampling}
        \EndIf

        \State \textbf{Estimate Pose:}
        \State Compute the estimated pose: $\hat{\mathbf{x}}^{(t)} = \sum_{i=1}^{N} w_i^{(t)} \mathbf{x}_i^{(t)}$
    \EndFor
\end{algorithmic}
\end{algorithm}




